Towards a Precision Measurement of Binary Black Holes Formation Channels Using Gravitational Waves and Emission Lines

The formation of compact objects-neutron stars, black holes, and supermassive black holes-and its connection to the chemical composition of the galaxies is one of the central questions in astrophysics. We propose a novel data-driven, multi-messenger technique to address this question by exploiting the inevitable correlation between gravitational waves and atomic/molecular emission line signals. For a fiducial probability distribution function $p(t_d)\propto t_d^{-\kappa}$ of time delays, this method can provide a measurement of the minimum delay time of $0.5$ Gyr and the power-law index $\kappa=1$ with a standard deviation $0.12$ (and $0.45$) and $0.06$ (and $0.34$), respectively from five years of LIGO-Virgo-KAGRA observation in synergy with SPHEREx line intensity mapping (and DESI emission-line galaxies). Such measurements will provide data-driven multi-messenger constraints on the delay time distribution which is currently not well known.

==> defs.tex <==

% math short cuts
\def\d{\partial}
\newcommand{\avg}[1]{\ensuremath{\left\langle \,#1\, \right\rangle}}
\def\dlP{\frac{\mathrm{d} \log P_m}{\mathrm{d}\log k}}
\def\dlM{\frac{\mathrm{d} \log \mathcal{M}}{\mathrm{d}\log k}}


\def\fnl{f_{\mathrm{NL}}^{\mathrm{loc}}}
\def\dq{\int \frac{\mathrm{d}^3q}{(2\pi)^3}}
\def\dpp{\int \frac{\mathrm{d}^3p}{(2\pi)^3}}
\def\dk{\int \frac{\mathrm{d}^3k}{(2\pi)^3}}
\def\eik{e^{i\vb{k}\cdot\vb{x}}}
\def\dlP{\frac{\mathrm{d} \log P}{\mathrm{d}\log k}}
\def\dlM{\frac{\mathrm{d} \log \mathcal{M}}{\mathrm{d}\log k}}



\def\la{\langle}
\def\ra{\rangle}
\def\dd{{\rm d}}
\def\ln{{\rm ln}}
\def\tr{{\rm tr}}
\def\det{{\rm det}}

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\ba{\begin{align}}
\def\ea{\end{\align}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}

\newcommand{\MpcOh}{ \,  \mathrm{Mpc}  \, h^{-1} }
\newcommand{\hOMpc}{ \,  \mathrm{Mpc}^{-1}  \, h  }
\newcommand{\nn}{ \nonumber }
\newcommand{\Msun}{ \,   M_{\odot}  {h}^{-1}   }

\newcommand{\fnl}{f_{\rm NL}}
\newcommand{\fnleq}{f_{\rm NL}^{\rm eq.}}
\newcommand{\fnlloc}{f_{\rm NL}^{\rm loc.}}
\newcommand{\fnlorth}{f_{\rm NL}^{\rm orth.}}

\def\bx{{\bf x}}
\def\bk{{\bf k}}
\def\bq{{\bf q}}
\def\kmq{{|\bk-\bq|}}
\def\iq{{\int_\bq}}
\def\bp{{\bf p}}

\def\cG{{\mathcal G}}
\def\cI{{\mathcal I}}
\def\cF{{\mathcal F}}
\def\cM{{\mathcal M}}













